Cyber-Physical Testbed Integrating RTAC with RTDS for Game-Theoretic Topology Control Under Load Altering Attacks

This paper introduces a cyber-physical testbed that integrates the Real-Time Digital Simulator (RTDS) with the Real-Time Automation Controller (RTAC) to enhance cybersecurity in electrical distribution networks. Focused on addressing vulnerabilities to cyber attacks, our testbed employs an advanced control algorithm developed in Python and executed through real-time controllers. Key to our approach is the seamless integration of the host PC machine, RTDS, and RTAC via the Modbus protocol. We present a game theory-based topology control strategy as an effective response to cyber attacks, specifically targeting smart meters. This testbed validates the efficacy of our method in fully eliminating voltage violations due to load altering attacks, showcasing substantial advancements in smart grid cybersecurity via the innovative use of RTDS and RTAC to simulate and counteract complex cyber threats.

==> Mendeley.tex <==
@online{raydocs,
  title = {Ray Documentation},
  author = {{Ray Team}},
  year = {2023},
  howpublished = {\url{https://www.ray.io}},
  note = {Accessed: 2023-10-01}
}

@online{rayintro,
  title = {Welcome to Ray! — Ray 2.7.1},
  author = {{Ray Team}},
  year = {2023},
  howpublished = {\url{https://docs.ray.io/en/latest/}},
  note = {Accessed: 2023-10-01}
}

@misc{raylibraries,
  title = {Ray Documentation | Libraries},
  author = {{Ray Team}},
  year = {2023},
  howpublished = {\url{https://www.ray.io/libraries}},
  note = {Accessed: 2023-10-01}
}

@misc{anyscale,
  title = {Ray Distributed Computing - Anyscale},
  author = {{Anyscale Team}},
  year = {2023},
  howpublished = {\url{https://www.anyscale.com/ray-distributed-computing}},
  note = {Accessed: 2023-10-01}
}


@inproceedings{fan2022powergym,
  title={Powergym: A reinforcement learning environment for volt-var control in power distribution systems},
  author={Fan, Ting-Han and Lee, Xian Yeow and Wang, Yubo},
  booktitle={Learning for Dynamics and Control Conference},
  pages={21--33},
  year={2022},
  organization={PMLR}
}


@inproceedings{li2021deep,
  title={Deep reinforcement learning based continuous volt-var optimization in power distribution systems with renewable energy resources},
  author={Li, Wenyun and Huang, Wei and Zhu, Tao and Wu, Minghe and Yan, Ziheng},
  booktitle={2021 IEEE Sustainable Power and Energy Conference (iSPEC)},
  pages={682--686},
  year={2021},
  organization={IEEE}
}

@article{gupta2022deep,
  title={Deep learning for optimal Volt/VAR control using distributed energy resources},
  author={Gupta, Sarthak and Chatzivasileiadis, Spyros and Kekatos, Vassilis},
  journal={arXiv preprint arXiv:2211.09557},
  year={2022}
}

@article{manna2022learning,
  title={Learning in continuous action space for developing high dimensional potential energy models},
  author={Manna, Sukriti and Loeffler, Troy D and Batra, Rohit and Banik, Suvo and Chan, Henry and Varughese, Bilvin and Sasikumar, Kiran and Sternberg, Michael and Peterka, Tom and Cherukara, Mathew J and others},
  journal={Nature communications},
  volume={13},
  number={1},
  pages={368},
  year={2022},
  publisher={Nature Publishing Group UK London}
}


@article{ming2023cooperative,
  title={Cooperative modular reinforcement learning for large discrete action space problem},
  author={Ming, Fangzhu and Gao, Feng and Liu, Kun and Zhao, Chengmei},
  journal={Neural Networks},
  volume={161},
  pages={281--296},
  year={2023},
  publisher={Elsevier}
}


@article{williams2022trajectory,
  title={Trajectory planning with deep reinforcement learning in high-level action spaces},
  author={Williams, Kyle R and Schlossman, Rachel and Whitten, Daniel and Ingram, Joe and Musuvathy, Srideep and Pagan, James and Williams, Kyle A and Green, Sam and Patel, Anirudh and Mazumdar, Anirban and others},
  journal={IEEE Trans. Aerospace and Electronic Systems},
  year={2022},
  publisher={IEEE}
}

@inproceedings{kanervisto2020action,
  title={Action space shaping in deep reinforcement learning},
  author={Kanervisto, Anssi and Scheller, Christian and Hautam{\"a}ki, Ville},
  booktitle={2020 IEEE conference on games (CoG)},
  pages={479--486},
  year={2020},
  organization={IEEE}
}

@inproceedings{espeholt2018impala,
  title={Impala: Scalable distributed deep-rl with importance weighted actor-learner architectures},
  author={Espeholt, Lasse and Soyer, Hubert and Munos, Remi and Simonyan, Karen and Mnih, Vlad and Ward, Tom and Doron, Yotam and Firoiu, Vlad and Harley, Tim and Dunning, Iain and others},
  booktitle={International conference on machine learning},
  pages={1407--1416},
  year={2018},
  organization={PMLR}
}

@article{haarnoja2018soft,
  title={Soft actor-critic algorithms and applications},
  author={Haarnoja, Tuomas and Zhou, Aurick and Hartikainen, Kristian and Tucker, George and Ha, Sehoon and Tan, Jie and Kumar, Vikash and Zhu, Henry and Gupta, Abhishek and Abbeel, Pieter and others},
  journal={arXiv preprint arXiv:1812.05905},
  year={2018}
}

@article{xu2020review,
  title={A review of cyber security risks of power systems: from static to dynamic false data attacks},
  author={Xu, Yan},
  journal={Protection and Control of Modern Power Systems},
  volume={5},
  number={1},
  pages={19},
  year={2020},
  publisher={Springer}
}

@article{schulman2017proximal,
  title={Proximal policy optimization algorithms},
  author={Schulman, John and Wolski, Filip and Dhariwal, Prafulla and Radford, Alec and Klimov, Oleg},
  journal={arXiv preprint arXiv:1707.06347},
  year={2017}
}


@article{cao2020reinforcement,
  title={Reinforcement learning and its applications in modern power and energy systems: A review},
  author={Cao, Di and Hu, Weihao and Zhao, Junbo and Zhang, Guozhou and Zhang, Bin and Liu, Zhou and Chen, Zhe and Blaabjerg, Frede},
  journal={Journal of modern power systems and clean energy},
  volume={8},
  number={6},
  pages={1029--1042},
  year={2020},
  publisher={SGEPRI}
}


@article{liu2022bi,
  title={Bi-level off-policy reinforcement learning for two-timescale volt/var control in active distribution networks},
  author={Liu, Haotian and Wu, Wenchuan and Wang, Yao},
  journal={IEEE Trans. Power Systems},
  volume={38},
  number={1},
  pages={385--395},
  year={2022},
  publisher={IEEE}
}


@article{zhang2020deep,
  title={Deep reinforcement learning based volt-var optimization in smart distribution systems},
  author={Zhang, Ying and Wang, Xinan and Wang, Jianhui and Zhang, Yingchen},
  journal={IEEE Trans. Smart Grid},
  volume={12},
  number={1},
  pages={361--371},
  year={2020},
  publisher={IEEE}
}

@article{gupta2023deep,
  title={Deep Learning for Scalable Optimal Design of Incremental Volt/VAR Control Rules},
  author={Gupta, Sarthak and Mehrizi-Sani, Ali and Chatzivasileiadis, Spyros and Kekatos, Vassilis},
  journal={IEEE Control Systems Letters},
  year={2023},
  publisher={IEEE}
}

@article{ma2023simplified,
  title={Simplified Deep Reinforcement Learning Based Volt-Var Control of Topologically Variable Power System},
  author={Ma, Qing and Deng, Changhong},
  journal={Journal of Modern Power Systems and Clean Energy},
  year={2023},
  publisher={SGEPRI}
}

@inproceedings{brugman2019cloud,
  title={Cloud based intrusion detection and prevention system for industrial control systems using software defined networking},
  author={Brugman, Jonathon and Khan, Mohammed and Kasera, Sneha and Parvania, Masood},
  booktitle={2019 Resilience Week (RWS)},
  volume={1},
  pages={98--104},
  year={2019},
  organization={IEEE}
}

@article{liu2011false,
  title={False data injection attacks against state estimation in electric power grids},
  author={Liu, Yao and Ning, Peng and Reiter, Michael K},
  journal={ACM Transactions on Information and System Security (TISSEC)},
  volume={14},
  number={1},
  pages={1--33},
  year={2011},
  publisher={ACM New York, NY, USA}
}

@article{kim2013topology,
  title={On topology attack of a smart grid: Undetectable attacks and countermeasures},
  author={Kim, Jinsub and Tong, Lang},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={31},
  number={7},
  pages={1294--1305},
  year={2013},
  publisher={IEEE}
}

@article{khan2020cyberphysical,
  title={The cyberphysical power system resilience testbed: Architecture and applications},
  author={Khan, Mohammed Masum Siraj and Palomino, Alejandro and Brugman, Jonathon and Giraldo, Jairo and Kasera, Sneha Kumar and Parvania, Masood},
  journal={Computer},
  volume={53},
  number={5},
  pages={44--54},
  year={2020},
  publisher={IEEE}
}



@inproceedings{huang2021real,
  title={Real-time power system simulation with hardware devices through dnp3 in cyber-physical testbed},
  author={Huang, Hao and Davis, C Matthew and Davis, Katherine R},
  booktitle={2021 IEEE Texas Power and Energy Conference (TPEC)},
  pages={1--6},
  year={2021},
  organization={IEEE}
}


@article{shariatzadeh2014real,
  title={Real-time implementation of intelligent reconfiguration algorithm for microgrid},
  author={Shariatzadeh, Farshid and Vellaithurai, Ceeman B and Biswas, Saugata S and Zamora, Ramon and Srivastava, Anurag K},
  journal={IEEE Trans. sustainable energy},
  volume={5},
  number={2},
  pages={598--607},
  year={2014},
  publisher={IEEE}
}

@inproceedings{biswas2013real,
  title={Real time testing and validation of Smart Grid devices and algorithms},
  author={Biswas, Saugata S and Shariatzadeh, Farshid and Beckstrom, Rory and Srivastava, Anurag K},
  booktitle={2013 IEEE Power \& Energy Society General Meeting},
  pages={1--5},
  year={2013},
  organization={IEEE}
}


@inproceedings{oyewumi2019isaac,
  title={Isaac: The idaho cps smart grid cybersecurity testbed},
  author={Oyewumi, Ibukun A and Jillepalli, Ananth A and Richardson, Philip and Ashrafuzzaman, Mohammad and Johnson, Brian K and Chakhchoukh, Yacine and Haney, Michael A and Sheldon, Frederick T and de Leon, Daniel Conte},
  booktitle={2019 IEEE Texas Power and Energy Conference (TPEC)},
  pages={1--6},
  year={2019},
  organization={IEEE}
}

@inproceedings{xiao2015development,
  title={Development of hardware-in-the-loop microgrid testbed},
  author={Xiao, Bailu and Starke, Michael and Liu, Guodong and Ollis, Ben and Irminger, Philip and Dimitrovski, Aleksandar and Prabakar, Kumaraguru and Dowling, Kevin and Xu, Yan},
  booktitle={2015 IEEE energy conversion congress and exposition (ECCE)},
  pages={1196--1202},
  year={2015},
  organization={IEEE}
}


@article{raschka2020machine,
  title={Machine learning in python: Main developments and technology trends in data science, machine learning, and artificial intelligence},
  author={Raschka, Sebastian and Patterson, Joshua and Nolet, Corey},
  journal={Information},
  volume={11},
  number={4},
  pages={193},
  year={2020},
  publisher={MDPI}
}


@inproceedings{xue2009socket,
  title={The socket programming and software design for communication based on client/server},
  author={Xue, Ming and Zhu, Changjun},
  booktitle={2009 Pacific-Asia Conference on Circuits, Communications and Systems},
  pages={775--777},
  year={2009},
  organization={IEEE}
}

@inproceedings{kornienko2021principles,
  title={Principles of securing RESTful API web services developed with python frameworks},
  author={Kornienko, DV and Mishina, SV and Shcherbatykh, SV and Melnikov, MO},
  booktitle={Journal of Physics: Conference Series},
  volume={2094},
  number={3},
  pages={032016},
  year={2021},
  organization={IOP Publishing}
}

@article{goldenberg2013accurate,
  title={Accurate modeling of Modbus/TCP for intrusion detection in SCADA systems},
  author={Goldenberg, Niv and Wool, Avishai},
  journal={international journal of critical infrastructure protection},
  volume={6},
  number={2},
  pages={63--75},
  year={2013},
  publisher={Elsevier}
}


@book{kusko2007power,
  title={Power quality in electrical systems},
  author={Kusko, Alexander and Thompson, Marc T},
  volume={23},
  year={2007},
  publisher={McGraw-Hill New York}
}

@inproceedings{selim2023deep,
  title={Deep Reinforcement Learning for Distribution System Cyber Attack Defense with DERs},
  author={Selim, Alaa and Zhao, Junbo and Ding, Fei and Miao, Fei and Park, Sung-Yeul},
  booktitle={2023 IEEE Power \& Energy Society Innovative Smart Grid Technologies Conference (ISGT)},
  pages={1--5},
  year={2023},
  organization={IEEE}
}

@misc{pymodbus,
  title = {PyModbus Documentation},
  year = {2023},
  howpublished = {\url{https://pymodbus.readthedocs.io/en/latest/}},
  note = {Accessed: 2023-12-03}
}

